BERRY: Bit Error Robustness for Energy-Efficient Reinforcement Learning-Based Autonomous Systems

Autonomous systems, such as Unmanned Aerial Vehicles (UAVs), are expected to run complex reinforcement learning (RL) models to execute fully autonomous position-navigation-time tasks within stringent onboard weight and power constraints. We observe that reducing onboard operating voltage can benefit the energy efficiency of both the computation and flight mission, however, it can also result in on-chip bit failures that are detrimental to mission safety and performance. To this end, we propose BERRY, a robust learning framework to improve bit error robustness and energy efficiency for RL-enabled autonomous systems. BERRY supports robust learning, both offline and on-board the UAV, and for the first time, demonstrates the practicality of robust low-voltage operation on UAVs that leads to high energy savings in both compute-level operation and system-level quality-of-flight. We perform extensive experiments on 72 autonomous navigation scenarios and demonstrate that BERRY generalizes well across environments, UAVs, autonomy policies, operating voltages and fault patterns, and consistently improves robustness, efficiency and mission performance, achieving up to 15.62% reduction in flight energy, 18.51% increase in the number of successful missions, and 3.43x processing energy reduction.

==> 2related_work.tex <==
\section{Related Work}
\label{sec:related}

\begin{comment}
\begin{itemize}
    \item Resilience of autonomous navigation
        \item Consider random bit-flip, transient errors, adversarial robustness.
        \item \textbf{Ours:} Profile on real low-voltage device and memory.
    \item Fault mitigation and protection methods
        \item Noise-aware training - supervised learning; hardware-based redundancy
        \item \textbf{Ours:} unsupervised learning, lightweight software-based method. We not only optimize compute perf/power, but also system perf/power.
\end{itemize}
\end{comment}


    
    % \subsection{Resilience Characterization in UAVs}
    % Several prior works have attempted to characterize the resilience of applications running on board a UAV.~\cite{venkatagiri2018swapprox} analyze the impact of several software approximations on the resilience of a video-summarization algorithm running on a UAV processor.~\cite{chan2020rlreliability} characterizes the reliability of several RL algorithms in terms of their inter-run variability, while~\cite{zhang2021robust,yang2022resilientQlearning} proposed techniques to train robust RL networks in the presence of adversarial perturbations, blackouts and other interferences. Unlike our proposed technique, none of these works tackle the problem of bit errors due to low voltages while running RL algorithms on UAVs or propose error-aware training techniques to mitigate their effects.


==> tabs/generalize_voltage.tex <==
\begin{table}[t!]
% \huge
\centering
\caption{\textbf{Comparison with Fixed Pattern Bit Error Training.} Training on an entirely fixed bit error pattern (FixPattBER) does not generalize to lower bit error rates, even though the bit errors are a subset of those during training. FixPattBER also fails to generalize to completely random bit errors. By contrast, \textsc{BERRY} generalizes to lower bit error rates and both fix ad random fault patterns.}
\renewcommand*{\arraystretch}{1.05}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cc|cc}
\hline
                                     & \multicolumn{2}{c|}{SuccRate (\%)} & \multicolumn{2}{c}{Flight Energy (J)} \\ \hline
\textbf{Evaluated on Fixed Pattern}    & $p$=0.1            & $p$=0.5           & $p$=0.1             & $p$=0.5             \\ \hline
FixPattBET $p$=0.5                     & 72.6             & 79.4            & 58.15             & 52.91             \\
\textsc{BERRY} $p$=0.5                          & \textbf{84.6}             & \textbf{79.2}            & \textbf{47.56}             & \textbf{53.04}             \\ \hline
\textbf{Evaluated on Random Pattern} & $p$=0.1            & $p$=0.5           & $p$=0.1             & $p$=0.5             \\ \hline
FixPattBET $p$=0.5                     & 73.0               & 52.8            & 57.34             & 66.76             \\
\textsc{BERRY} $p$=0.5                          & \textbf{84.8}             & \textbf{79.0}              & \textbf{46.91}             & \textbf{52.98}             \\ \hline
\end{tabular}
}
\label{tab:gen_vol}
\vspace{-3pt}
\end{table}

==> tabs/rlbet_result_summary.tex <==
\begin{table}[t!]
\huge
\centering
\caption{\textbf{Bit Error Training (BET).} Average task success rate and quality-of-flight evaluated at various voltage and bit error rates. BET increase robustness. Operating at lower voltage, BET reduces system-level flight time energy usage, and improves number of missions.}
\renewcommand*{\arraystretch}{1.05}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc|c|cccc}
\hline
\multicolumn{2}{c|}{Low-voltage Operation}                                                                             & Robustness                                                   & \multicolumn{4}{c}{Quality of Flight}                                                                                                                                                                                                                  \\ \hline
\begin{tabular}[c]{@{}c@{}}Voltage \\ (V)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Bit Error \\ Rate $p$ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Success \\ Rate (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Flight \\ Time (s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Flight \\ Distance (m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Flight \\ Energy (J)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Num. of\\ Missions\end{tabular} \\ \hline

1       & 0                        & 88.4              & 6.81            & 14.89               & 53.19             & 55.35            \\ \hline
0.6              & 1.96$\times$10^${-6}$                 & 88.0              & 6.51            & 14.93               & 47.23             & 62.05            \\
0.59             & 1.38$\times$10^${-5}$                 & 89.2              & 6.48            & 14.86               & 46.66             & 63.66            \\
0.58             & 8.23$\times$10^${-5}$                 & 89.0              & 6.46            & 14.91               & 46.41             & 63.85            \\
0.57             & 4.22$\times$10^${-4}$                 & 88.8              & 6.45            & 14.96               & 46.22             & 63.98            \\
0.56             & 1.87$\times$10^${-3}$                 & 88.6              & 6.42            & 14.94               & 45.80             & 64.42            \\
0.55             & 7.25$\times$10^${-3}$                 & 88.6              & 6.39            & 14.94               & 45.38             & 65.01            \\
\textbf{0.54}             & \textbf{2.47$\times$10$^{-2}$}                 & 88.4              & \textbf{6.35}            & \textbf{14.91}               & \textbf{44.88}             & \textbf{65.59}   \\
0.53             & 7.49$\times$10^${-2}$                 & 86.2              & 6.67            & 15.71               & 46.90             & 61.20            \\
0.52             & 2.03$\times$10^${-1}$                 & 83.4              & 7.03            & 16.58               & 49.14             & 56.52            \\
0.51             & 4.98$\times$10^${-1}$                 & 79.0              & 7.61            & 18.03               & 52.98             & 49.66            \\
0.5              & 1.11                     & 74.4              & 8.18            & 19.46               & 56.62             & 43.75            \\
0.475            & 5.80                     & 63.2              & 9.09           & 21.84              & 61.96             & 33.96            \\
0.45            & 20.36                     & 50.4              & 10.11           & 24.52              & 67.83             & 24.74            \\\hline
\end{tabular}
}
\label{tab:rlbet_summary}
\vspace{-3pt}
\end{table}



